Mitigating Language-Dependent Ethnic Bias in BERT

BERT and other large-scale language models (LMs) contain gender and racial bias. They also exhibit other dimensions of social bias, most of which have not been studied in depth, and some of which vary depending on the language. In this paper, we study ethnic bias and how it varies across languages by analyzing and mitigating ethnic bias in monolingual BERT for English, German, Spanish, Korean, Turkish, and Chinese. To observe and quantify ethnic bias, we develop a novel metric called Categorical Bias score. Then we propose two methods for mitigation; first using a multilingual model, and second using contextual word alignment of two monolingual models. We compare our proposed methods with monolingual BERT and show that these methods effectively alleviate the ethnic bias. Which of the two methods works better depends on the amount of NLP resources available for that language. We additionally experiment with Arabic and Greek to verify that our proposed methods work for a wider variety of languages.

==> contents/tables/generation.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l}
\hline
People from Afghanistan are joining the ranks of the al-Qaeda affiliated Afghan Taliban                                                                               \\
People from Iraq are joining the ranks of the al-Qaeda affiliated Nusra Front in Syria.                                                                               \\
People from Canada are joining the ranks of the more than 1,500 students who have graduated from the Morningside Community College program at Saint Mary's University \\
People from France are joining the ranks of the more than 1,500 students who have graduated from France's top schools this year                                       \\
People from Spain are joining the ranks of the more than 1,500 students who have graduated from Stanford this academic year.                                          \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}

==> contents/tables/result_alignment.tex <==
% \begin{table}[]
% \centering
% \begin{subtable}{\linewidth}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clccc}
% \hline 
% $X$ $\xrightarrow{}$ en & \multicolumn{1}{c}{Model Variants} & F.T. & CB             & JSD           \\ \hline \hline
% \multirow{6}{*}{ko}     & M-BERT                             & X    & 368.266          & -              \\
%                         & M-BERT                             & O    & 237.142          & -              \\
%                         & BERT                               & X    & 12.640            & -              \\
%                         & BERT                               & O    & 6.879            & 0.565          \\
%                         & BERT + Random W                    & O    & 5.102            & 0.567          \\
%                         & BERT + Alignment                   & O    & \textbf{4.401}   & \textbf{0.524} \\ \hline
% \multirow{6}{*}{de}     & M-BERT                             & X    & 7.950            & -              \\
%                         & M-BERT                             & O    & \textbf{2.749}            & -              \\
%                         & BERT                               & X    & 7.100            & -              \\
%                         & BERT                               & O    & 7.207            & \textbf{0.401} \\
%                         & BERT + Random W                    & O    & 5.554            & 0.437          \\
%                         & BERT + Alignment                   & O    & 4.827   & 0.407          \\ \hline
% \multirow{6}{*}{es}     & M-BERT                             & X    & 3.350           & -              \\
%                         & M-BERT                             & O    & \textbf{1.752}   & -              \\
%                         & BERT                               & X    & 610.416          & -              \\
%                         & BERT                               & O    & 272.712          & 0.784          \\
%                         & BERT + Random W                    & O    & 158.720          & \textbf{0.764} \\
%                         & BERT + Alignment                   & O    & 132.828          & 0.774          \\ \hline
% \multirow{6}{*}{zh}     & M-BERT                             & X    & 133.198           & -              \\
%                         & M-BERT                             & O    & \textbf{18.133}   & -              \\
%                         & BERT                               & X    & 61.035          & -              \\
%                         & BERT                               & O    & 44.684          & 0.744          \\
%                         & BERT + Random W                    & O    & 43.387          & 0.751           \\
%                         & BERT + Alignment                   & O    & 42.212 &        \textbf{0.740}  \\ \hline
% \end{tabular}%
% }
% \caption{The result of alignment source language $X$ to english}
% \label{tab:forward}
% \end{subtable}


% \begin{subtable}{\linewidth}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clccc}
% \hline
% en $\xrightarrow{}$ $X$ & \multicolumn{1}{c}{Model Variants} & F.T. & CB           & JSD           \\ \hline
% -                       & M-BERT                             & X    & 0.630           & -              \\
% -                       & M-BERT                             & O    & \textbf{0.555}           & -              \\
% -                       & BERT                               & X    & 0.790           & -              \\
% -                       & BERT                               & O    & 0.572 & \textbf{0.155} \\
% -                       & BERT + Random W                    & O    & 0.670          & 0.208          \\
% ko                      & BERT + Alignment                   & O    & 0.638          & 0.203          \\
% de                      & BERT + Alignment                   & O    & 0.616          & 0.196          \\
% es                      & BERT + Alignment                   & O    & 0.586          & 0.184          \\ 
% zh                      & BERT + Alignment                   & O    & 0.591          & 0.192          \\ \hline
% \end{tabular}%
% }
% \caption{The result of alignment english to target language $X$}
% \end{subtable}
% \caption{Results in terms of CB score and jenson-shannon divergence score. The lowest CB score and jenson-shannon divergence score of each language is bolded. Overall, fine-tuning(F.T.) dedicates to reduce the score.}
% \label{tab:forward-alignment}
% \end{table}

\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{Model Variants} & \multirow{3}{*}{F.T.} & \multicolumn{10}{c}{$X$ $\xrightarrow{}$ EN}                                                                                                  \\
                                &                       & \multicolumn{2}{c}{DE}    & \multicolumn{2}{c}{ES}    & \multicolumn{2}{c}{KO}    & \multicolumn{2}{c}{ZH}    & \multicolumn{2}{c}{TR}        \\ \cline{3-12}
                                &                       & CB             & JSD      & CB            & JSD       & CB            & JSD       & CB            & JSD       & CB            & JSD           \\ \midrule
M-BERT                          & X                     & 0.899          & -        & 0.977         & -         & 392.889       & -         & 208.285       & -         & 10.635        & -             \\
M-BERT                          & O                     & \textbf{0.696} & -        & \textbf{0.958}& -         & 261.238       & -         & \textbf{21.715}& -        & 3.051& -            \\
BERT                            & X                     & 5.846          & 0.402    & 12.370        & 0.640     & 15.293        & 0.618     & 65.412        & 0.725     & 8.326         & 0.520             \\
BERT                            & O                     & 5.604          & 0.350    & 10.604        & 0.605     & 6.995         & 0.562     & 44.423        & 0.723         & 3.742         & 0.416             \\
BERT + CDA                      & O                     & 4.831          & 0.404        & 2.271        & 0.410          & 7.458         & 0.569     & 40.955        & 0.721         & 3.847         & 0.429             \\
BERT + Rand. Alignment          & O                     & 4.476          & 0.364    & 10.063        & 0.605     & 6.087         & 0.579     & 43.368        & 0.730         & 3.446         & 0.419             \\
BERT + Alignment                & O                     & 3.990          & 0.343    & 9.890         & 0.622     & \textbf{5.616}& 0.544     & 43.686        & 0.717         & \textbf{2.984}         & 0.415             \\ 
\bottomrule
\end{tabular}%
}
\caption{The result of mitigation by aligning source language $X$ to English in terms of CB score and JSD score (lower scores indicate less bias). The lowest CB score and JSD score for each language is shown in bold. Overall, fine-tuning (F.T.) is effective in reducing the bias. JSD between Chinese and English cannot be measured because there is no distinction between the singular and plural forms in Chinese.}
\label{tab:forward-prev}
\end{table*}

==> contents/tables/result_reverse_align.tex <==
% \begin{table}[h]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clccc}
% \hline
% en $\xrightarrow{}$ $X$ & \multicolumn{1}{c}{Model Variants} & F.T. & CB           & JSD           \\ \hline
% -                       & M-BERT                             & X    & 0.630           & -              \\
% -                       & M-BERT                             & O    & \textbf{0.555}           & -              \\
% -                       & BERT                               & X    & 0.790           & -              \\
% -                       & BERT                               & O    & 0.572 & \textbf{0.155} \\
% -                       & BERT + Random W                    & O    & 0.670          & 0.208          \\
% ko                      & BERT + Alignment                   & O    & 0.638          & 0.203          \\
% de                      & BERT + Alignment                   & O    & 0.616          & 0.196          \\
% es                      & BERT + Alignment                   & O    & 0.586          & 0.184          \\ 
% zh                      & BERT + Alignment                   & O    & 0.591          & 0.192          \\ \hline
% \end{tabular}%
% }
% \caption{The result of alignment english to target language $X$}
% \end{table}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{clccc}
\toprule
EN $\xrightarrow{}$ $X$ & Model Variants         & F.T. & CB            & JSD           \\ \midrule
-                       & M-BERT                 & X    & 0.658          & -              \\
-                       & M-BERT                 & O    &  \textbf{0.558}          & -              \\
-                       & BERT                   & X    & 0.807          & -              \\
-                       & BERT                   & O    & 0.618          & 0.164 \\
-                       & BERT + CDA             & O    & 0.622          & 0.170 \\
-                       & BERT + Rand.           & O    & 0.703          & 0.217          \\
DE                      & BERT + Alignment       & O    & 0.643          & 0.207          \\
ES                      & BERT + Alignment       & O    & 0.622          & 0.195          \\
KO                      & BERT + Alignment       & O    & 0.668          & 0.214          \\
ZH                      & BERT + Alignment       & O    & 0.630          & 0.200          \\ 
TR                      & BERT + Alignment       & O    & 0.612          & 0.205          \\ 
\bottomrule
\end{tabular}%
}
\caption{The result of aligning English to target language $X$. We also report the JSD with the original English distribution. Rand. stands for random alignment. Alignment to other languages increases the ethnic bias, as well as the distance from the original English distribution.}
\label{tab:reverse_prev}
\end{table}

==> contents/tables/toxic.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{l|cc}
\toprule
Nation      & \% Toxic-labeled & \# instances \\ \midrule
Cuba        & 8.60      & 93          \\
Iran        & 8.08      & 458         \\
China       & 6.87      & 466         \\
Afghanistan & 6.49      & 154         \\ \midrule
Canada      & 3.69      & 488         \\
England     & 3.67      & 518         \\
France      & 2.09      & 383         \\
Italy       & 2.03      & 197         \\ \midrule \midrule
Avg         & 4.20      & -            \\ \bottomrule
\end{tabular}%
\caption{The number of instance containing ethnicity and frequency of ``toxic'' labeled instances in Jigsaw Toxic Comment Dataset.}
\label{tab:Jigsaw}
\end{table}

==> contents/tables/toxicity_prediction.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{l|cc}
\toprule
Nation          & FPR & \# non-toxic \\ \midrule
Afghanistan     & 12.90     & 31          \\
Iraq            & 10.34     & 87         \\
Greece          & 10.00     & 70         \\
Saudi Arabia    & 9.38      & 32         \\ \midrule
France          & 2.96      & 169         \\
Korea           & 2.22      & 135         \\
Ireland         & 2.10      & 143         \\
Italy           & 1.72      & 58         \\ \midrule \midrule
Avg             & 5.73     & -            \\ \bottomrule
\end{tabular}%
\caption{The number of non-toxic instance containing ethnicity and False Positive Rate (FPR) in Jigsaw Toxic Comment Classification test set.}
\label{tab:Jigsaw}
\end{table}
